DepthBench: Measuring How Residual Connections Enable More Computational Depth

Depth is a natural way to increase the computational capacity in Transformers, yet the contribution of deeper layers can diminish as depth grows larger. Recent approaches enhance normalization (\text{e.g.}, LayerNorm Scaling) or residual connections (\text{e.g.}, mHC, AttnRes) to enable better information flow and depth utilization. However, it remains unclear whether they truly translate increased architectural depth into effective computational depth, and whether their reported gains stem from better access to information across depth, or unaccounted-for confounding factors. In this paper, we introduce \textbf{DepthBench}, a controlled benchmark for studying computational depth across various architectures. We systematically vary the width--depth aspect ratio ($d_{\text{model}}/n_{\text{layer}}$) from shallow--wide to deep--narrow shapes, while keeping the model size and pre-training recipe fixed. Across 10 representative architectures, we find that the benefit of allocating more capacity to depth is strongly architecture-dependent. Standard Pre-LN and most of its norm- and scaling-based variants provide little benefit and can even degrade performance as models become deeper and narrower, whereas HC and Full AttnRes improve consistently even at extreme deep shapes. These gains extend beyond pre-training loss and consistently translate into improved domain-specific performance and effective computation. Controlled layer-level analyses further show that the gains of HC and Full AttnRes are associated with more effective utilization of additional layers, revealing distinct mechanisms of computational depth across architectures. Overall, our results identify residual connection design as a key determinant of whether depth can serve as a meaningful scaling axis by enabling additional architectural depth to translate into effective computation.

==> figures_old/hc_mhc_transport_geometry.tex <==
% Replaces the standalone aspect-ratio rank figure in the mHC discussion.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/hc_mhc_transport_geometry.pdf}
    \caption{\textbf{Residual transport in HC and mHC.}
    \textbf{(a)} Effective rank across aspect ratios, with shapes $(L,d)$ below
    each tick. Effective rank is the exponential of the entropy of the
    normalized singular values.
    \textbf{(b)} Mean absolute cosine similarity between propagated stream
    directions in $L=32$ models.
    \textbf{(c)} Singular values of their full residual products, normalized
    by the largest.
    Statistics are averaged over sampled held-out FineWeb-Edu data;
    bands and error bars show 95\% document-bootstrap intervals.}
    \label{fig:hc_mhc_residual_rank}
\end{figure}


==> tables_old/architecture_sketch.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.18}
    \caption{
        Overview of residual update mechanisms for the architectures \cite{attnres}.
        Architectures differ primarily in how layer $\ell$ receives and aggregates
        information from preceding depths. \textit{Weight}: whether the mixing coefficients are fixed or input-dependent (dynamic). \textit{Source}: which earlier representations layer $\ell$ can access.
    }
    \label{architecture_sketch}
    \label{tab:architectures}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llll}
        \toprule
        \textbf{Method}
        & \textbf{Update rule}
        & \textbf{Weight}
        & \textbf{Source} \\
        \midrule

        \multicolumn{4}{l}{\textbf{\textit{Baseline}}} \\[-1pt]
        \hspace{1em}Pre-LN \cite{pre-ln}
        &
        $h_\ell
        =
        h_{\ell-1}
        +
        F_\ell(\mathrm{LN}(h_{\ell-1}))$
        &
        Fixed
        &
        $h_{\ell-1}$ \\

        \addlinespace[2pt]
        \midrule

        \multicolumn{4}{l}{\textbf{\textit{LayerNorm variants}}} \\[-1pt]
        \hspace{1em}Sandwich-LN \cite{sandwich-ln1}
        &
        $h_\ell
        =
        h_{\ell-1}
        +
        \mathrm{LN}_{\mathrm{out}}
        \!\left(
            F_\ell(\mathrm{LN}_{\mathrm{in}}(h_{\ell-1}))
        \right)$
        &
        Fixed
        &
        $h_{\ell-1}$ \\

        \hspace{1em}LNS \cite{lns}
        &
        $h_\ell
        =
        h_{\ell-1}
        +
        F_\ell\!\left(
            \frac{1}{\sqrt{\ell}}
            \mathrm{LN}(h_{\ell-1})
        \right)$
        &
        Fixed
        &
        $h_{\ell-1}$ \\

        \hspace{1em}DeepNorm \cite{deepnorm}
        &
        $h_\ell
        =
        \mathrm{LN}\!\left(
            \alpha h_{\ell-1}
            +
            F_\ell(h_{\ell-1})
        \right)$
        &
        Fixed
        &
        $h_{\ell-1}$ \\

        \hspace{1em}KEEL \cite{keel}
        &
        $h_\ell
        =
        \mathrm{LN}\!\left(
            \alpha h_{\ell-1}
            +
            F_\ell(\mathrm{LN}(h_{\ell-1}))
        \right)$
        &
        Fixed
        &
        $h_{\ell-1}$ \\

        \addlinespace[2pt]
        \midrule

        \multicolumn{4}{l}{\textbf{\textit{Multi-stream residuals} }} \\[-1pt]
        \hspace{1em}HC \cite{hc}
          &            
          $H_\ell             
          = H_{\ell-1}A_\ell
          + F_\ell\!\left(\mathrm{LN}(H_{\ell-1}\alpha_\ell)\right)
            \beta_\ell^\top$      
          &         
          Dynamic
          &                    
          $m$ residual streams \\
  \hspace{1em}mHC \cite{mhc}
  &
  $\begin{aligned}                          
  H_\ell                       
  &= H_{\ell-1}\mathrm{Sinkhorn}(\widetilde A_\ell)
   + F_\ell\!\left(\mathrm{LN}(H_{\ell-1}\sigma(\widetilde\alpha_\ell))\right)
     2\sigma(\widetilde\beta_\ell^\top)
  \end{aligned}$
  &                       
  Dynamic
  &                                
  $m$ residual streams \\
        \addlinespace[2pt]
        \midrule

        \multicolumn{4}{l}{\textbf{\textit{Cross-layer access} }} \\[-1pt]

        \multirow{2}{*}{\hspace{1em}AttnRes \cite{attnres}}
        &
        $\textit{Full:}\quad
        h_\ell
        \propto
        \sum_{i=0}^{\ell-1}
        \phi(w_\ell,v_i)v_i,
        \quad
        v_0 = h_1,\;
        v_{i \geq 1} = f_i(h_i)$
        &
        Dynamic
        &
        $[h_1,\ldots,h_{\ell-1}]$\vspace{0.10em}  \\

        &
        $\textit{Block:}\quad
        h_\ell
        \propto
        \sum_{i=0}^{n-1}
        \phi(w_\ell,v_i)v_i
        +
        \phi(w_\ell,v_n^{j})v_n^{j}$
        &
        Dynamic
        &
        $[v_0,\ldots,v_{n-1},v_n^{j}]$ \vspace{0.40em} \\ 

        %\vspace{1em}

        \hspace{1em}{MoDA (Pre-LN)} \cite{moda}
          &
          $h_\ell
          = h_{\ell-1}
          + \mathrm{MoDA}_\ell\!\left(
              \mathrm{LN}(h_{\ell-1});\mathcal C_{<\ell}
            \right)$
          &
          Dynamic
          &
          $\bigl[
              h_{\ell-1,\le t};
              h_{0,t},\ldots,h_{\ell-2,t}
          \bigr]$\\

        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables_old/main_model_configs.tex <==
\begin{table}[t]
\centering
\caption{Main model configurations across different width--depth aspect ratios.}
\label{tab:aspect_ratio_configs}
\small
\begin{tabular}{rrrrrrrrr}
\toprule
Layers & Hidden & Intermediate & Heads & Head Dim. & Aspect Ratio & Backbone Size & Total Size & Total Diff. \\
\midrule
16 & 1216 & 3248 & 16 & 76 & 76.00 & 284M & 407M & +0.28\% \\
20 & 1120 & 2992 & 16 & 70 & 56.00 & 301M & 414M & +2.14\% \\
24 & 1024 & 2736 & 16 & 64 & 42.67 & 302M & 405M & 0.00\% \\
28 & 960  & 2560 & 16 & 60 & 34.29 & 310M & 406M & +0.21\% \\
32 & 896  & 2400 & 16 & 56 & 28.00 & 309M & 399M & -1.49\% \\
\bottomrule
\end{tabular}
\end{table}m

==> tables_old/optimal_learning_rate.tex <==
\begin{table}[t]
\centering
\caption{Optimal learning rate across architectures.}
\label{tab:optimal_lr}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{*{10}{c}}
\toprule
 Pre-LN & Sandwich-LN & LNS & DeepNorm & KEEL & MoDA & Full AttnRes & Block AttnRes & HC & mHC  \\
\midrule
 $2 \times 10^{-3}$ & $2 \times 10^{-3}$ & $1 \times 10^{-2}$ & $1 \times 10^{-3}$ & $2 \times 10^{-3}$ & $2 \times 10^{-3}$ & $2 \times 10^{-3}$ & $2 \times 10^{-3}$ & $2 \times 10^{-3}$ & $2 \times 10^{-3}$ \\
\bottomrule
\end{tabular}
}
\end{table}
